Relative Pose for Nonrigid Multi-Perspective Cameras: The Static Case

Multi-perspective cameras with potentially non-overlapping fields of view have become an important exteroceptive sensing modality in a number of applications such as intelligent vehicles, drones, and mixed reality headsets. In this work, we challenge one of the basic assumptions made in these scenarios, which is that the multi-camera rig is rigid. More specifically, we are considering the problem of estimating the relative pose between a static non-rigid rig in different spatial orientations while taking into account the effect of gravity onto the system. The deformable physical connections between each camera and the body center are approximated by a simple cantilever model, and inserted into the generalized epipolar constraint. Our results lead us to the important insight that the latent parameters of the deformation model, meaning the gravity vector in both views, become observable. We present a concise analysis of the observability of all variables based on noise, outliers, and rig rigidity for two different algorithms. The first one is a vision-only alternative, while the second one makes use of additional gravity measurements. To conclude, we demonstrate the ability to sense gravity in a real-world example, and discuss practical implications.

==> modificationSuggestions.tex <==
%\documentclass[10pt,twocolumn,letterpaper]{article}
%\begin{document}

\section{modificationSuggestions}
\subsection{discussion_with_Laurent_about_modification}
1. tile

2. abstract, change the order
   we are looking at relative pose problem, consider static or stationary case
   solve relative under deformation
   under use of simple cantilever model to express deformation, already be able to prove observability of variables based on noise, outliers and rig rigidity
   soften our claim, static relative pose estimation, keep statement observe gravity
   
3. intro, mention application from cantilever model? (-Min) primarily a theoretical study if deformability observes additional variables. not to claim cantilever has practical use, but prove certain facts about observability of the physics. 
add a discussion session at the end of the paper to discuss about the practical usuage of this. cantilever, though simple, sufficient to prove blabla, cranes, airplane wings,  serves as important first step, then more competent work use complete physical model following this. list a few cases with deformability, study with simple model
fundamental work
emphasize: not just 2 or 4 cams system, extendable to any various physical models, length, location, rigidities, etc. not only point mass? but also different load forms, like distributed force, or gravity of the bar itself?

4. theory, (a) equation number, (b) add one reference from the textbook

5. syntheticExp, font size of the figures

6. realExp, different rigidities

7. a paragraph describe the the model, though simpla but a strong indication of using physical model to target nonrigid system



\subsection{Previous_Min's_suggestions_on_modification}

             Target for 3DV, revise the manuscript to make it stronger
Modify the title, tailor it specific to cantilever-bar
Therefore, in the introduction part, we should emphasize the application from cantilever model, restricting the reviewers from requiring it to other applications.
It is the start of a series research works, we will extend it to more complicated model, which include the heat, atmosphere, age, even wind, etc.
Font size in the figures, enlarge.
Explain more detail about the algorithm, no-lacking-of-readability or repeatability to the reviewer
More sets of real-experiment data. Unfortunately, we only have two pointgrey, maybe we stick to the two-camera system, but add several different rigidities.  
emphasize that it can be extended to any number of camera system, with different rigidities and lengths, and physical properties.

\subsection{Reviewers'Comments}

[Meta-review] Consolidation Report explaining the decision for the submission to authors. Must be based on the reviews, rebuttal, and the discussions with reviewers and AC-Triple.The paper initially received diverging ratings: 1 strong accept, 1 borderline and 1 weak reject. The strengths of the paper were the introduction of non-rigid multi-camera systems compatible with RANSAC, supportive experimental results, and clear technical presentation of the proposed work. The weaknesses pointed by the reviewers were limited real-world experiments (R1), missing mathematical derivation of the algorithm (R2), being tailored to a specific simple configuration (R3), and that the cause of deformation can be various. The authors provided the answers to these issues. After the rebuttal, R1 remained strongly supportive to the work, but the other reviewers lowered their ratings to weak reject and borderline reject. The AC checked all reviews and the feedback, participated in the discussion, and agrees with the negative evaluation. The rejection decision was also discussed in and approved by the AC triplet.

\subsubsection{Reviewer #1}
Questions
1. [Reviewer Guidelines] By taking this review assignment and checking on "I agree" below, I acknowledge that I have read and understood the reviewer guidelines (https://iccv2023.thecvf.com/reviewer.guidelines-362000-2-16-20.php).
Agreement accepted
2. [Large Language Model (LLM) Ethics] ICCV’23 does not allow the use of Large Language Models or online chatbots such as ChatGPT in any part of the reviewing process. There are two main reasons: - Reviewers must provide comments that faithfully represent their original opinions on the papers being reviewed. It is unethical to resort to Large Language Models (e.g., an offline system) to automatically generate reviewing comments that do not originate from the reviewer’s own opinions. - Online chatbots such as ChatGPT collect conversation history to improve their models. Therefore their use in any part of the reviewing process would violate the ICCV confidentiality policy (https://iccv2023.thecvf.com/ethics.for.reviewing.papers-362100-2-16-21.php). Herewith I confirm that I have not used an online chatbot such as ChatGPT in preparing the review. This review reflects my own opinions, and no parts were generated by an automatic system.I agree
4. [Summary] Describe the key ideas, experiments, and their significance (preferably in 5-7 sentences).This paper presents a method for handling non-rigid deformations of a multi-camera rig cause by gravity. They show that even with no overlap the gravity direction and rig deformation can be computed from point correspondences, given the appropriate system motion (largely motion constraints set out in previous papers). The paper models the cameras as being mounted to flexible bars which do not stretch or shrink but only bend. Three methods are compared to compute the relative pose of the multi-camera system (MCS). One, which assumes no bend even though the MCS does bend, two which optimizes for the gravity vector after generating a six point solution, and three which uses the measured gravity vector to provide two degrees of freedom so requiring only four point correspondences. They show that the four point method is more accurate with a fairly flexible bar. As the bar is made stiffer the difference between the rigid system assuming six-point rigid method and the other two methods decreases, matching what one would expect. In addition to these synthetic experiments, the paper presents experiments on a real two camera system on a cantilever bar. The real experiments show the same trend as the synthetic results, with the four point algorithm outperforming the other two methods, as expected.
5. [Strengths] Consider the aspects of key ideas, experimental or theoretical validation, writing quality, and data contribution (if relevant). Explain clearly why these aspects of the paper are valuable. Short, unjustified review is NOT OK.The paper is clearly written. The mathematics lay out the problem in its entirety so that the result can be reproduced.
While it is a simplified non-rigid system model, the demonstration that any flexible mounting model can be handled in a RANSAC framework is a positive step forward.
The discussions of future work including finite element methods for more complex systems point the way to more general solutions.
The experiments are thorough and show the method is effective. Results match one's intuition about the problem, which is a nice touch.
6. [Weaknesses] Consider the aspects of key ideas, experimental or theoretical validation, writing quality, and data contribution (if relevant). Explain clearly why these are weak aspects of the paper. Short, unjustified review is NOT OK. For example: a comment saying that this has been done before must be accompanied by specific reference(s) and an explanation of how they overlap; a comment saying that the experiments are insufficient to validate the claims should be accompanied by explanations of what exactly is missing; not achieving state-of-the-art, or not surpassing prior methods, is not sufficiently a weakness, unless this comment is justified; a comment of “lack of novelty” should be carefully justified, and novelty could involve new insights/understandings or new discoveries/observations, not just new technical methods.It's not clear in figure 9 what (a) (b) and (c) are in the plots. Please indicate which of the surfaces represent which. I can guess but it should be shown in the figure.
It would be interesting to see the real experiment include different rigidity bars, from completely stiff to flexible as shown. That would further demonstrate the effectiveness of the method and back up the synthetic results.
7. [Paper rating]1. Strong accept
8. [Recommendation confidence]Very confident: I am an expert on this topic.
9. [Justification of rating] Provide detailed justification of your rating. It should involve how you weigh the strengths and weaknesses of the paper.This paper solves an important, realistic problem encountered in multi-camera systems. Non-rigidity of mounting is a general problem that requires a solution. As a community we have been assuming it was not an issue with our methods because we didn't have an effective solution. We'd simply strive to make the system as physically rigid as possible. This has its limits, particularly when system weight is constrained. This paper points the community in a better direction.
10. [Additional comments] Minor suggestions, questions, corrections, etc. that can help the authors improve the paper, if any.line 727 "augments" -> "increases" Using augments in a sentence this way is pretty unusual. Augments means to increase the amount of something by adding to it. Someone or something has to be doing the augmenting. "Bob augments his income by driving for Uber" is correct, while "Driving for Uber causes Bob's income to augment" is not.
11. [Dataset contributions] Does a paper claim a dataset release as one of its scientific contributions?No
12. [Post-Rebuttal Recommendation] Give your final rating for this paper. Don't worry about poster vs oral. Consider the input from all reviewers, the authors' feedback, and any discussion. (Will be visible to authors after author notification)1. Strong Accept
13. [Post-Rebuttal Justification] Justify your post-rebuttal assessment. Acknowledge any rebuttal and be specific about the final factors for and against acceptance that matter to you. (Will be visible to authors after author notification)
I read the other reviews, the rebuttal and discussion. I still believe this is a significant paper worthy of publication at ICCV. Handling non-rigid camera mountings is an interesting subject that has not gotten enough attention. The paper demonstrates one method for modeling these systems with both synthetic and real experiment showing that it works well.

\subsubsection{Reviewer #2}

Questions
1. [Reviewer Guidelines] By taking this review assignment and checking on "I agree" below, I acknowledge that I have read and understood the reviewer guidelines (https://iccv2023.thecvf.com/reviewer.guidelines-362000-2-16-20.php).Agreement accepted
2. [Large Language Model (LLM) Ethics] ICCV’23 does not allow the use of Large Language Models or online chatbots such as ChatGPT in any part of the reviewing process. There are two main reasons: - Reviewers must provide comments that faithfully represent their original opinions on the papers being reviewed. It is unethical to resort to Large Language Models (e.g., an offline system) to automatically generate reviewing comments that do not originate from the reviewer’s own opinions. - Online chatbots such as ChatGPT collect conversation history to improve their models. Therefore their use in any part of the reviewing process would violate the ICCV confidentiality policy (https://iccv2023.thecvf.com/ethics.for.reviewing.papers-362100-2-16-21.php). Herewith I confirm that I have not used an online chatbot such as ChatGPT in preparing the review. This review reflects my own opinions, and no parts were generated by an automatic system.I agree
4. [Summary] Describe the key ideas, experiments, and their significance (preferably in 5-7 sentences).This paper proposes a new camera model, named Non-Rigid Multi-Perspective Camera (NR-MPC), which allows a deformation of the support structures of a multi-camera rig. Since the generalized relative pose problem of the NR-MPCs is highly non-linear, this paper assumes a static case where the camera-rig is composed of cantilever bars and is influenced by only gravity. Under the cantilever model, this paper derives two solutions to the generalized relative pose problem, and also discusses the degenerate cases of this model. In the synthetic experiment, the robustness against image noise and rigidity noise is first investigated, then, the robustness against outliers and gravity noise, and the computational time are reported. Finally, the proposed solvers are tested on a real data where two cameras are mounted on two cantilever bars for each.
5. [Strengths] Consider the aspects of key ideas, experimental or theoretical validation, writing quality, and data contribution (if relevant). Explain clearly why these aspects of the paper are valuable. Short, unjustified review is NOT OK.- The proposed camera model, NR-MPC, is novel and could be helpful in a wide range of CV applications, especially for robot/UAV navigation.
- The cantilever model is introduced to describe the non-rigid transformation between a camera and the supported body.
- The proposed theory constrains the two-view geometry of non-overlapping MPCs.
- The degenerate configurations are roughly discussed.
- The survey of relevant literature is comprehensive.
6. [Weaknesses] Consider the aspects of key ideas, experimental or theoretical validation, writing quality, and data contribution (if relevant). Explain clearly why these are weak aspects of the paper. Short, unjustified review is NOT OK. For example: a comment saying that this has been done before must be accompanied by specific reference(s) and an explanation of how they overlap; a comment saying that the experiments are insufficient to validate the claims should be accompanied by explanations of what exactly is missing; not achieving state-of-the-art, or not surpassing prior methods, is not sufficiently a weakness, unless this comment is justified; a comment of “lack of novelty” should be carefully justified, and novelty could involve new insights/understandings or new discoveries/observations, not just new technical methods.A major weakness of this paper is the lack of clarity about the derivation of the mathematical equations in Sec.3.2, which provides the theoretical background of the new concept. For example, it is unclear how to derive the equations in ll.362-368, and there is no explanation for the denominator Ei*Ii. Lines 505-508 do not describe the definition of vector angles (what is Wij^T(B_g){...}?). The manuscript omits both the mathematical details and sufficient information needed to reproduce the proposed method. Due to this, it is difficult to validate the correctness of the experiments. In addition, the displayed equations are barely numbered, which does not follow the author guidelines, losing the readability.

Another weakness is that the bendability of bars is ignored in the first solution. As the authors mention, this situation coincides with that of the 6-point method [35]. Therefore, it is not an appropriate scenario for NR-MPCs.
7. [Paper rating]4. Weak reject
8. [Recommendation confidence]Very confident: I am an expert on this topic.
9. [Justification of rating] Provide detailed justification of your rating. It should involve how you weigh the strengths and weaknesses of the paper.This paper proposes a new concept for the geometric problem of computer vision, which could be of broad interest to the community. However, the manuscript needs more clarity and readability so that the readers can validate the theoretical aspect.
10. [Additional comments] Minor suggestions, questions, corrections, etc. that can help the authors improve the paper, if any.- Font size in all figures is too small.
- What are the ground-truth camera motions in the real data experiment? Moreover, it is questionable to say "verified the applicability" in ll.753-755 from the large estimation error (0.67 rad = 38 deg) in the gravity direction.
11. [Dataset contributions] Does a paper claim a dataset release as one of its scientific contributions?No
12. [Post-Rebuttal Recommendation] Give your final rating for this paper. Don't worry about poster vs oral. Consider the input from all reviewers, the authors' feedback, and any discussion. (Will be visible to authors after author notification)5. Weak Reject
13. [Post-Rebuttal Justification] Justify your post-rebuttal assessment. Acknowledge any rebuttal and be specific about the final factors for and against acceptance that matter to you. (Will be visible to authors after author notification)I keep my rating because the rebuttal is not convincing enough.

1) ll.035-036 in the rebuttal does not show an appropriate reference to explain the math equations in ll.365-368 in the manuscript.

2) ll.057-068 in the rebuttal does not answer the cause of the significant estimation error in the gravity direction. In general, error distributions should be almost equal for all parameters under appropriate modeling. The result where the error is biased only in the gravity direction suggests that the double approximation (the cantilever model and the assumptions in Sec. 3.3) is not appropriate.

From my viewpoint, the current form tries to start with a difficult situation. For example, a quick remedy to clarify the second issue is to use IMUs and make the gravity direction of each camera (and the body frame) known. Since IMUs are already popularized, it is a more realistic situation than the case where an initial gravity direction of the body frame is only measurable (ll. 466-468 in the manuscript).

\subsubsection{Reviewer #3}

Questions
1. [Reviewer Guidelines] By taking this review assignment and checking on "I agree" below, I acknowledge that I have read and understood the reviewer guidelines (https://iccv2023.thecvf.com/reviewer.guidelines-362000-2-16-20.php).Agreement accepted
2. [Large Language Model (LLM) Ethics] ICCV’23 does not allow the use of Large Language Models or online chatbots such as ChatGPT in any part of the reviewing process. There are two main reasons: - Reviewers must provide comments that faithfully represent their original opinions on the papers being reviewed. It is unethical to resort to Large Language Models (e.g., an offline system) to automatically generate reviewing comments that do not originate from the reviewer’s own opinions. - Online chatbots such as ChatGPT collect conversation history to improve their models. Therefore their use in any part of the reviewing process would violate the ICCV confidentiality policy (https://iccv2023.thecvf.com/ethics.for.reviewing.papers-362100-2-16-21.php). Herewith I confirm that I have not used an online chatbot such as ChatGPT in preparing the review. This review reflects my own opinions, and no parts were generated by an automatic system.I agree
4. [Summary] Describe the key ideas, experiments, and their significance (preferably in 5-7 sentences).The paper presents a method to compute the relative pose of two multi-perspective cameras considering the case where two non-overlapping cameras are connected by a beam that deforms. The paper presents a method that consider the deformation caused by the weight of the two cameras. The paper presents experiments on synthetic datasets as well as on a real-world scenario showing the robustness and effectiveness of the proposed method.
5. [Strengths] Consider the aspects of key ideas, experimental or theoretical validation, writing quality, and data contribution (if relevant). Explain clearly why these aspects of the paper are valuable. Short, unjustified review is NOT OK.Overall, I think the paper is well written, well motivated, and the execution of the experiments is well done. Below are more details:
1. Clarify of the paper is good. I think thee narrative is quite clear, the Figures are illustrative and help follow the notation and derivation. I think the paper can be reproduced given its good clarity.
2. The problem of extending the study of non-central cameras to the non-rigidity assumption is a tough problem but an interesting one. In practice, the extension of these cameras can very impactful, especially in newer AR/VR and robotic devices that can experiment deformations over time given heat, usage, etc. Because a solution to this problem is important, I support the investigation in this direction.
6. [Weaknesses] Consider the aspects of key ideas, experimental or theoretical validation, writing quality, and data contribution (if relevant). Explain clearly why these are weak aspects of the paper. Short, unjustified review is NOT OK. For example: a comment saying that this has been done before must be accompanied by specific reference(s) and an explanation of how they overlap; a comment saying that the experiments are insufficient to validate the claims should be accompanied by explanations of what exactly is missing; not achieving state-of-the-art, or not surpassing prior methods, is not sufficiently a weakness, unless this comment is justified; a comment of “lack of novelty” should be carefully justified, and novelty could involve new insights/understandings or new discoveries/observations, not just new technical methods.While I value the clarity and importance of the problem, I find the derivation very specific to a single configuration of non-overlapping cameras. I only have one major concern on this front: the described approach is limited to one configuration. See details below:
1. Derivation of the proposed method is tailored to a simple configuration of the cameras: two non-overlapping cameras attached with a long beam. First, while this is a good start, I think the title of the paper is quite misleading. As it sounds more general than what the proposed method actually solves. Second, it is not clear from the text why this configuration is important to study. Which applications comply w/ the setting of having two non-overlapping cameras attached by a single beam and that its weight deforms the beam connecting them? How can this method be extended to more cameras?
2. In many applications where multiple cameras are used, the deformations are not caused mainly by the weight of the cameras. Consider for instance AR/VR headsets. The weights of those cameras are quite small and a deformation of the rig is not mainly due to weight reasons. In those devices, mainly heat, usage, and other factors affect the relative poses of the array of cameras. I think the paper is lacking a justification about focusing only one one reason for deformations. It would've been very informative to know these reasons over other factors that also deform the array of cameras.
7. [Paper rating]3. Borderline
8. [Recommendation confidence]Very confident: I am an expert on this topic.
9. [Justification of rating] Provide detailed justification of your rating. It should involve how you weigh the strengths and weaknesses of the paper.While I like the problem addressed here and the clarity of the paper is good, I am not finding a convincing argument justifying the derivation of the method for a single camera array: two cameras connected by a single beam that can deform as a consequence of the weight of the cameras.
10. [Additional comments] Minor suggestions, questions, corrections, etc. that can help the authors improve the paper, if any.Please make plots in Figure 11 larger. They are hard to parse.
11. [Dataset contributions] Does a paper claim a dataset release as one of its scientific contributions?No
12. [Post-Rebuttal Recommendation] Give your final rating for this paper. Don't worry about poster vs oral. Consider the input from all reviewers, the authors' feedback, and any discussion. (Will be visible to authors after author notification)4. Borderline Reject
13. [Post-Rebuttal Justification] Justify your post-rebuttal assessment. Acknowledge any rebuttal and be specific about the final factors for and against acceptance that matter to you. (Will be visible to authors after author notification)Unfortunately, the rebuttal did not change my perception of the paper. Here are the reasons:
1. I find that the title and abstract over-sell the generality of the solution. Unfortunately, the solution is tailored to a single configuration. I think a more interesting paper would include more than two cameras and demonstrate that the framework would scale to any number of cameras.
2. I think the motivation of the presented configuration is not solid enough. I think the configuration is quite unique with perhaps a handful of applications. Thus, I think the paper may not trigger much interest in the community.
In sum, I think the research is tackling an interesting problem, but the solution is not general enough for me to recommend acceptance. I think the paper can revise the paper to make it stronger for the next computer vision venue.

%\end{document}
